Finding All {\epsilon}-Good Arms in Stochastic Bandits

The pure-exploration problem in stochastic multi-armed bandits aims to find one or more arms with the largest (or near largest) means. Examples include finding an {\epsilon}-good arm, best-arm identification, top-k arm identification, and finding all arms with means above a specified threshold. However, the problem of finding all {\epsilon}-good arms has been overlooked in past work, although arguably this may be the most natural objective in many applications. For example, a virologist may conduct preliminary laboratory experiments on a large candidate set of treatments and move all {\epsilon}-good treatments into more expensive clinical trials. Since the ultimate clinical efficacy is uncertain, it is important to identify all {\epsilon}-good candidates. Mathematically, the all-{\epsilon}-good arm identification problem presents significant new challenges and surprises that do not arise in the pure-exploration objectives studied in the past. We introduce two algorithms to overcome these and demonstrate their great empirical performance on a large-scale crowd-sourced dataset of 2.2M ratings collected by the New Yorker Caption Contest as well as a dataset testing hundreds of possible cancer drugs.

==> comparison_to_topk.tex <==
\section{Comparison to top $k$}
This is a quick note comparing the complexity of \st2 to \texttt{LUCB1} by \cite{kalyanakrishnan2012pac}. In all cases, for both algorithms, let $\gamma = 0$.

In the case of top-$k$, gaps are defined as: 
$$
\Delta_i^k=
\begin{cases}
\mu_i - \mu_{k+1}, & \text{ if } 1\leq i \leq k \\
\mu_k - \mu_{i}, & \text{ if } k+1\leq i \leq n
\end{cases}
$$
Further, define $c = \frac{\mu_k + \mu_{k+1}}{2}$.
\cite{kalyanakrishnan2012pac} show that
$$\Delta_i^k / 2 \leq |\mu_i - c| \leq \Delta_i^k.$$

Hence, we may compare to $\frac{\mu_k + \mu_{k+1}}{2}$ as opposed to $\mu_k$ or $\mu_{k+1}$ and pay only a constant factor. We are interested in the setting where $G_\epsilon = \mu_k$. Let 
$$\epsilon = \mu_1 - \frac{\mu_k + \mu_{k+1}}{2}.$$
Then 
$$\mu_1 - \epsilon = \frac{\mu_k + \mu_{k+1}}{2}.$$
Furthermore, 
$$\alpha_\epsilon = \beta_\epsilon = \mu_k - \frac{\mu_k + \mu_{k+1}}{2} = \frac{\mu_k - \mu_{k+1}}{2}.$$

For arms in $G_\epsilon^c$ (arms $k+1, \cdots, n$), 
$$ \frac{1}{(\mu_1 - \epsilon - \mu_i)^2} = \frac{1}{\left(\frac{\mu_k + \mu_{k+1}}{2} - \mu_i\right)^2},$$
matching their contribution to the complexity of returning the top-$k$ arms up to a constant, given in Theorem~6 of \cite{kalyanakrishnan2012pac}, the upper bound on the complexity of \texttt{LUCB}.

For arms in $G_\epsilon$, Theorem~\ref{thm:st2_complexity}, their contribution to the sample complexity is
\begin{align*}
\max\left\{\frac{1}{\left(\frac{\mu_k + \mu_{k+1}}{2} - \mu_i\right)^2}, \frac{1}{\left(\mu_1 + \alpha_\epsilon - \mu_i\right)^2}, \frac{1}{\left(\mu_1 + \beta_\epsilon - \mu_i\right)^2} \right\} \\ = \max\left\{\frac{1}{\left(\frac{\mu_k + \mu_{k+1}}{2} - \mu_i\right)^2}, \frac{1}{\left(\mu_1 + \frac{\mu_k - \mu_{k+1}}{2} - \mu_i\right)^2} \right\}
\end{align*}
For $i$ such that $\mu_i \leq \frac{\mu_1 + \mu_k}{2}$
\[\max\left\{\frac{1}{\left(\frac{\mu_k + \mu_{k+1}}{2} - \mu_i\right)^2}, \frac{1}{\left(\mu_1 + \frac{\mu_k - \mu_{k+1}}{2} - \mu_i\right)^2} \right\} = \frac{1}{\left(\frac{\mu_k + \mu_{k+1}}{2} - \mu_i\right)^2}, \]
equal to that arm's contribution to the top-$k$ bound. For $i$ such that $\mu_i \geq \frac{\mu_1 + \mu_k}{2}$, \begin{align*}
    \mu_1 + \frac{\mu_k - \mu_{k+1}}{2} - \mu_i & \geq \mu_1 + \frac{\mu_k - \mu_{k+1}}{2} - \frac{\mu_1 + \mu_k}{2} \\
    & = \frac{2\mu_1 - \mu_1 - \mu_k + \mu_k - \mu_{k+1}}{2} \\
    & = \frac{\mu_1 - \mu_{k+1}}{2} \\
    & \geq \frac{1}{2}\left(\mu_1 - \frac{\mu_k + \mu_{k+1}}{2} \right).
\end{align*}
Hence, their contribution to all-$\epsilon$ is at most $\frac{4}{\left( \mu_1 - \frac{\mu_k + \mu_{k+1}}{2}\right)^2}$.
Note that
\begin{align*}
    \mu_i - \frac{\mu_k + \mu_{k+1}}{2} 
    & \leq \mu_1 - \frac{\mu_k + \mu_{k+1}}{2} 
\end{align*}
Hence, for such arms, their contribution to the bound in top-$k$ is at least
$$\frac{1}{\left( \mu_1 - \frac{\mu_k + \mu_{k+1}}{2}\right)^2}.$$

Combining all pieces, we see that the complexity of \st2 when $\epsilon = \mu_1 - \frac{\mu_k + \mu_{k+1}}{2}$ is within a constant factor of that of \texttt{LUCB1}. 

==> conclusion.tex <==
\section{Conclusion}
In this paper, we propose the question of returning a set containing all $\epsilon$-good arms and none worse than $(\epsilon+\gamma)$-good for a slack variable $\gamma$. We propose an algorithm \texttt{EAST} for general $\gamma$ that enjoys good practical performance as well as a second method, \texttt{FAREAST} that draws on ideas from sparse signal detection and is optimal in the case that $\gamma=0$. Additionally, we show how to extend \texttt{EAST} to consider thresholds defined by general Lipschitz functions of the highest mean, and this allows us to provide a method for returning multiplicative $\epsilon$-good arms, defined by a percentage of the highest mean. The algorithms and theoretical guarantees herein are a strong first step towards this problem, and motivate other settings and theoretical questions.
% but there are several open theoretical questions related to finding all $\epsilon$-good arms. 
% First, the sample complexity of \texttt{FAREAST} \ref{thm:fareast_complex} includes several moderate complexity terms which are independent of $\delta$. In practical settings, these terms greatly affect the complexity unless $\delta$ is very small. It is unknown whether these terms are necessary. This relates to the classic question of detection versus estimation in a sparse signal as studied in \cite{donoho2004higher} amongst others. In the context of this work, one can use results such as \cite{simchowitz2017simulator} to show that any algorithm to \emph{return} an arm with a positive mean requires $O(n\beta^{-2} + \beta^{-2}\log(1/\delta))$ samples, and we use this idea to remove arms in $G_\epsilon^c$ in \texttt{FAREAST}. However, if one only wishes to declare that there \emph{exists} an arm with a positive mean, it is unknown if the $O(n\beta^{-2})$ term is necessary. 
First, it is unknown if the lower bound in Theorem \ref{thm:inst_lower} is achievable by an algorithm that gives a high probability guarantee on its sample complexity. 
The sample complexities \texttt{FindPos} as well as the method in \cite{mannor2004sample} are only bounded in expectation and do not hold in high probability. 
% Finally, this work motivates several related questions. 
Furthermore, it may be interesting to consider functions of more means such as the highest $k$ or even all $n$ capturing the questions studied in \cite{zhang2019adaptive, zhangadaptive}. 
%\cite{zhang2019adaptive, zhangadaptive} study problems where a threshold can be defined as a special functions of all $n$ means, and a method that can split arms due to more general functions of the means could encapsulate both of these as well as ours. 
Finally, in many real world settings, each arm may be defined by a $d$-dimensional feature vector. One could similarly consider a linear bandits extension to finding all $\epsilon$-good arms. 




% \textbf{Open questions and motivating areas for further study}
% \begin{enumerate}
%     \item can the moderate confidence terms be removed in this problem (or can we show they are necessary?)
%     \item how to do this with linear bandits
%     \item searching over functions of $\mu_1$, more complex sets of arms where this tradeoff of explore the threshold exploit the threshold show up. 
%     \item analyzing bandit problems from the notion of high-probability sample complexity. Currently, Kauffman tells us how to do this in expectation, and Mannor and Tsisiklis tell us how to do this for algs with probability $1$ sample complexities via the notion of ``path-wise sample complexity.'' As this paper indicates, guarantees for these different settings can be difference and even involve different terms ($\alpha$ vs. $\beta$). In real world problems, we may need more control over sample complexity that expected complexity, but probability $1$ may be too stringent. For instance in the Mannor and Tsitsiklis case (and in positive mean) this leads to an additional factor of $n$ samples that are necessary (on the $\log(1/\delta)$ term!). 
% \end{enumerate}

==> mod_ST2.tex <==
\begin{algorithm}[h]
\caption{The \st2 Algorithm \label{alg:st2}}
\begin{algorithmic}[1]
\Require{$\epsilon, \delta > 0$, Instance $\nu = \{i: \mu_i\}$ of $n$ $1$-subGaussian arms}
\State{Pull each arm once, initialize $T_i \leftarrow 1$, update $\hat{\mu}_i, \ell_i, u_i$ for each $i \in \{1, 2, \ldots, n\}$}
\State{Find the best empirical arm  and compute the set of empirical good arms  $\widehat{G}_\epsilon$}
\State{Find the arm with the highest upper bound $i^\ast(t) = \arg \max \hat{u}_i(t)$, set $L^\ast(t) = \ell_{i^\ast}(t) - \epsilon, U^\ast = u_{i^\ast}(t) - \epsilon$}
\While{$\exists i: [\ell_i(t), u_i(t)] \cap [L^\ast(t), U^\ast(t)] \neq \emptyset $}
%\State{Pull arm $i_1(t) = \arg\max_i u_i(t)$}
\If{$\exists \ i \in \widehat{G}_{\epsilon} \text{ s.t. } \ell_i(t) < U^\ast(t)$}
\State{Pull arm $i_1(t) = \arg\min_{i \in \widehat{G}_{\epsilon}}  \ell_i(t)$, update $T_{i_1}, \hat{\mu}_{i_1}, \ell_{i_1}, u_{i_1}$}
\EndIf
\If{$\exists \ i \in \widehat{G}_{\epsilon}^c \text{ s.t. } u_i(t) > L^\ast(t)$}
\State{Pull arm $i_2(t) = \arg\max_{i \in \widehat{G}_{\epsilon}^c} u_i(t)$, update $T_{i_2}, \hat{\mu}_{i_2}, \ell_{i_2}, u_{i_2}$}
\EndIf
\If{$T_{i^\ast} < \max\{T_{i_1}, T_{i_2}\}$}
% \State{Initialize a set of arms $\mathcal{J} \leftarrow \{i^\ast\}$}
% \Repeat
% \State{$\mathcal{J} \leftarrow \mathcal{J} \cup \{i \notin \mathcal{J}: u_i(t) > \max\{u_j(t): j \in \mathcal{J}\}\}$}
% \State{$\mathcal{J} \leftarrow \mathcal{J} \setminus \{i \in \mathcal{J}: u_i(t) < \max\{l_j(t): j \in \mathcal{J}\}\}$}
% \State{Pull each arm $j \in \mathcal{J}$, update $T_j, \hat{\mu}_j, \ell_j, u_j$}
% \Until{$\max\{T_j : j \in \mathcal{J}\}$ is equal to $\max\{T_{i_1}, T_{i_2}\}$}
\State{Pull arm $i^\ast$, update $T_{i^\ast}, \hat{\mu}_{i^\ast}, \ell_{i^\ast}, u_{i^\ast}$}
\State{Update $i^\ast \leftarrow \arg\max u_i$ and corresponding $L^\ast(t), U^\ast(t)$}
\EndIf
%\State{Update bounds and empirical means}
\EndWhile
\Return The set of good arms $\widehat{G}_{\epsilon}$
\end{algorithmic}
\end{algorithm}

\textbf{Correctness} in the good event $\cE$ is due to the stopping condition. Denoting $i^\ast = \arg\max u_i$, when all bounds are correct, the highest mean $\mu_1 \in [\ell_{i^\ast}, u_{i^\ast}]$. Hence $\mu_1 - \epsilon \in [L^\ast, U^\ast]$, implying that finally all the arms are classified (correctly under $\cE$) as either good or bad. 

\textbf{Sample complexity:} by adding the maximum number of samples taken from each arm under $\cE$.

\textbf{Claim:} For any arm~$i$, if $T_i$ is the number of samples taken from it, then under the good event $\cE$
\begin{equation*}
\mu_i - 2C_{\delta/n}(T_i) 
\leq \ell_i \leq \mu_i \leq u_i 
\leq \mu_i + 2C_{\delta/n}(T_i).
\end{equation*}
This is because when all bounds are correct $u_i = \hat{\mu}_i + C_{\delta/n}(T_i) \geq \mu_i \implies \hat{\mu}_i \geq \mu_i - C_{\delta/n}(T_i)$, and hence $\ell_i = \hat{\mu}_i - C_{\delta/n}(T_i) \geq \mu_i - 2C_{\delta/n}(T_i)$.

A bad arm $i \in G_\epsilon^c$ is stopped sampling once its $u_i < L^\ast$ or when $u_i < \mu_{k+1}$, the bad arm with the highest mean. 


, which is ensured when
$\mu_i + 2C_{\delta/n}(T_i) < \mu_{i^\ast} - 2C_{\delta/n}(T_{i^\ast}) - \epsilon \leq \ell_{i^\ast} - \epsilon$. By definition $u_{i^\ast} \geq u_1$

==> mod_conf_lower_bound.tex <==
\section{Lower bounds in the moderate confidence regime}\label{sec:mod_conf_lb}
In this section, we prove a tighter lower bound that includes \emph{moderate confidence} terms independent of the value of $\delta$ similar to those that appear in the upper bound on the sample complexity of \texttt{FAREAST}, Theorem~\ref{thm:fareast_complex}. To do so, we begin be proving a lower bound on the following problem, referred to as \emph{spike-detection}. 

\subsection{Lower bounds for spike-detection}\label{sec:1spike_detect}
Fix $n \in \mathbb{N}$, $\beta > 0$, and $\delta > 0$.
Consider a set $\nu$ of $n$ Gaussian random variables such that there exists a spike $i^\ast \in [n]$ with $\rho_{i^\ast} = {\cal N}(\beta,1)$ whose index is unknown and chosen uniformly at random.
\marginpar{what do you mean by random here?}. 
The remaining $\rho_i = {\cal N}(0,1) \ \forall \ i \in [n]\backslash\{i^\ast\}$. Refer to this set of $n$ distributions collectively as an instance $\nu$.

\textbf{The $1$-Spike detection problem:} Given an instance as described above where $i^\ast$ is sampled uniformly from $[n]$ and unknown. We refer to $i^\ast$ as the \emph{spike}.
By sampling individual distributions, a player wishes to return an index $\hat{i}$ such that with probability greater than $1-\delta$, $\hat{i} = i^\ast$. 

\begin{lemma}\label{lem:1spike_kauf}
Fix $n$ and $\beta$ and consider a set $\nu$ of $n$ Gaussian random variables 
% \marginpar{and the rest are mean 0?} 
such that for a uniformly random chosen $i^\ast \in [n]$, $\rho_{i^\ast} = {\cal N}(\beta, 1)$ and $\rho_{i} = {\cal N}(0, 1)$ for all $i \neq i^\ast$. Any algorithm that correctly returns $i^\ast$ with probability at least $1-\delta$, samples $\rho_{i^\ast}$
\marginpar{I am not sure what the guarantee is?} 
$$ \frac{2}{\beta^2}\log(1/2.4\delta)$$
times in expectation.
\end{lemma}

\begin{remark}
Note that this gives a lower bound on the complexity of $1$-spike detection. 
\end{remark}

\begin{proof}
Consider the oracle setting where the value of $i^\ast$ is known and the algorithm only seeks to confirm that $\rho_i \neq {\cal N}(0, 1)$. Lemma $1$ of \cite{kaufmann2016complexity} implies that any $\delta$-PAC algorithm requires at least $ \frac{2}{\beta^2}\log(1/2.4\delta)$
samples in expectation. 
\end{proof}

The above bound controls the number of samples that any algorithm must gather from $i^\ast$. However, the proof considered an oracle setting where the value of $i^\ast$ is known, and one only wishes to confirm that $\rho_{i^\ast} \neq {\cal N}(0, 1)$ with probability at least $1-\delta$. To lower bound the number of samples drawn from $[n]\backslash \{i^\ast\}$, we need significantly more powerful tools. In particular, to rule out trivial algorithms that always output a fixed index, we consider a permutation model, as in \cite{mannor2004sample, simchowitz2017simulator, katz2019true, chen2017nearly}. Informally, we consider an additional expectation in the lower bound over a random permutation $\pi$ of the arms where $\pi$ is sampled uniformly from the set of all permutations. In particular, we with use a \emph{Simulator} argument, as in \cite{simchowitz2017simulator, katz2019true}. In what follows, we will let $\pi: [n] \rightarrow [n]$ denote a permutation selected uniformly at random from the set of $n!$ permutations. For instance $\nu$, let $\pi(\nu)$ denote the permuted instance such that the $i^\text{th}$ distribution is mapped to $\pi(i)$, by a slight overloading of the definition of $\pi(\cdot)$. In what follows, we proceed similarly to the proof of Theorem 1 in \cite{katz2019true}. 

\begin{theorem}\label{thm:simulator}
Fix $n$, $\beta$, and $\delta < 1/16$ and consider a set $\nu$ of $n$ Gaussian random variables such that for a uniformly random chosen $i^\ast \in [n]$, $\rho_{i^\ast} = \N(\beta, 1)$. Let $\pi$ be a uniformly chosen permutation of $[n]$ and $\pi(\nu)$ be the permutation applied to instance $\nu$. Let $T$ be the random variable denoting the total number of samples at termination by an algorithm. Any $\delta$-PAC algorithm to detect $\pi(i^\ast)$ on $\pi(\nu)$ requires
$$\E_{\pi}\E_{\pi(\nu)}\left[T\right] \geq \frac{1}{16} \frac{n-1}{\beta^2}$$
samples in expectation from arms in $[n]\backslash \{i^\ast\}$.
\end{theorem}

\begin{remark}
Note that this serves as a lower bound on the complexity of $1$-spike detection, and also applies to the positive effect detection problem. 
\end{remark}

\begin{proof}
Fix a permutation $\pi$. Let $\pi(\nu)$ be the permutation applied to $\nu$ and $\pi(i)$ be the index of $i$ under the permuted instance, $\pi(\nu)$. Let $\A$ be any algorithm that detects and returns $\pi(i^\ast)$ on $\pi(\nu)$ with probability at least $1-\delta$. We will take $\P_\A$ and $\E_\A$ to denote probability and expectation with respect any internal randomness in $\A$. 
Throughout, we will take $\rho_i = \N(\mu_i, 1)$ to denote the $i^\text{th}$ distribution of $\nu$ and note that $\mu_i$ is either $0$ if $i \neq i^\ast$ or $\beta$ if $i = i^\ast$.

% Chen argument: not correct beacuse need to average over permutations
% Next, for $i \neq i^\ast$, again consider the event $E$. By assumption, this happens with probability at least $1-\delta$. Construct the alternate instance $\nu'$ where $\rho_i = \N(\beta, 1)$. On $\nu'$, $i$ and $i^\ast$ share the same distribution. Therefore, due to the randomness in the choice of $i^\ast$, the probability of $E$ is $1/2$ since $i$ and $i^\ast$ are indistinguishable. Again by applying the same Lemma, we have that
% $$2\E_\nu[N_i]\beta^2 \geq d(1-\delta, 1/2) \geq (1 -\delta) \log(2) \geq \log(2)/2$$
% where $d(\cdot, \cdot)$ is the binary entropy function and the final inequality follows from $\delta \leq 1/2$. Repeating this argument for each $i \neq i^\ast$ and combining with the previous completes the proof. 
% \end{proof}

Fix $k \neq i^\ast$. To bound the necessary number of samples for arm $k$, we turn to the Simulator \cite{simchowitz2017simulator}. We begin by defining an alternate instance $\nu' = \{\rho'_1, \cdots, \rho'_n\}$ as \marginpar{$\nu'_k$ maybe?}
$$
\rho'_{j}=
\begin{cases}
\rho_j, & j \neq i^\ast\\
\rho_k, & j = i^\ast\\
\rho_{i^\ast}, & j = k\\
\end{cases}
$$
\noindent Note that $\nu'$ is identical to $\nu$ except that the distributions of $i^\ast$ and $k$ are swapped. Let $E$ be the event that $\A$ returns $\pi(i^\ast)$.
We may bound the total variation distance between the joint distribution on $\A \times \pi(\nu)$ and $\A \times \pi(\nu')$ as 

\begin{eqnarray*}
TV(\P_{\A \times \pi(\nu)}, \P_{\A \times \pi(\nu')}) & = & \sup_{A} \left| \P_{\A \times \pi(\nu)}(A) - \P_{\A \times \pi(\nu')}(A)\right| \\
&\geq & \left| \P_{\A \times \pi(\nu)}(E) - \P_{\A \times \pi(\nu')}(E)\right| \\
&\geq & 1 - 2\delta
\end{eqnarray*}
where $E$ is the event defined above that $\A$ returns $\pi(i^\ast)$.
%and the supremum is taken over events $A$ in the filtration generated by $\A$ playing on the instance $\pi(\nu)$.

Let $\Omega_t$ denote the multiset of the transcript of samples up to time $t$ and define the events 
$$W_j(\Omega_t) := \left\{\sum_{i \in \Omega_t}\1(i=j) \leq \tau \right\}$$
for a $\tau$ to be defined later. With the definitions of $W_j(\Omega_t)$, we define a simulator $\text{Sim}(\nu, \Omega_t)$ with respect to $\nu$. Let $\text{Sim}(\nu, \Omega_t)_i$ denote the distribution of arm $i$ on $\text{Sim}(\nu, \Omega_t)$. 

$$
\text{Sim}(\nu, \Omega_t)_{j} = 
\begin{cases}
\rho_j, & \text{ if } j \notin \{i^\ast, k\} \\
\rho_j, & \text{ if } j \in \{i^\ast, k\} \text{ and } W_{i^\ast}(\Omega_t) \cap W_{k}(\Omega_t)\\
\rho_{i^\ast}, & \text{ if } j \in \{i^\ast, k\} \text{ and } (W_{i^\ast}(\Omega_t) \cap W_{k}(\Omega_t))^c\\
\end{cases}
$$
Furthermore, we define $\text{Sim}(\nu', \Omega_t)$ with respect to $\nu'$ as 

$$
\text{Sim}(\nu', \Omega_t)_{j} = 
\begin{cases}
\rho_j', & \text{ if } j \notin \{i^\ast, k\} \\
\rho_j', & \text{ if } j \in \{i^\ast, k\} \text{ and } W_{i^\ast}(\Omega_t) \cap W_{k}(\Omega_t)\\
\rho_{i^\ast}, & \text{ if } j \in \{i^\ast, k\} \text{ and } (W_{i^\ast}(\Omega_t) \cap W_{k}(\Omega_t))^c\\
\end{cases}
$$
For ease of notation, let $\text{Sim}(\pi(\nu), \Omega_t)$ be the same simulator defined on $\pi(\nu)$ and with respect to events $W_{\pi(i^\ast)}(\Omega_t)$ and $W_{\pi(k)}(\Omega_t)$. Note that in the simulator of $\nu'$, if $(W_{i^\ast}(\Omega_t) \cap W_{k}(\Omega_t))^c$ is true, then $i^\ast$ and $k$ draw samples according to instance $\nu$ not $\nu'$. 

\begin{definition}(Truthfulness of an event $W$, \cite{katz2019true})
For an algorithm $\A$, we say that an event $W$ is truthful on a simulator $\text{Sim}(\eta)$ with respect to an instance $\eta$ if for all events $E$ in the filtration ${\cal F}_T$ generated by playing algorithm $\A$ on instance $\eta$
$$\P_\eta(E\cap W) = \P_{\text{Sim}(\eta)}(E \cap W)$$
\end{definition}

By our definition of both simulators, if $(W_{i^\ast}(\Omega_t) \cap W_{k}(\Omega_t))^c$ is true, then $\text{Sim}(\nu, \Omega_t)_{i} = \text{Sim}(\nu', \Omega_t)_{i} \ \forall i \in [n]$. Contrarily, if $W_{i^\ast}(\Omega_t) \cap W_{k}(\Omega_t)$ is true, then $\text{Sim}(\nu, \Omega_t) = \nu$ and $\text{Sim}(\nu', \Omega_t) = \nu'$. Similarly, on $W_{\pi(i^\ast)}(\Omega_t) \cap W_{\pi(k)}(\Omega_t)$, $\text{Sim}(\pi(\nu), \Omega_t) = \pi(\nu)$ and $\text{Sim}(\pi(\nu'), \Omega_t) = \pi(\nu')$. Therefore, by the proof of Theorem~1 of \cite{katz2019true}, $W_{\pi(k)}(\Omega_t)$ is truthful on $\text{Sim}(\pi(\nu), \Omega_t)$ and $ W_{\pi(i^\ast)}(\Omega_t)$ is truthful on $\text{Sim}(\pi(\nu'), \Omega_t)$. \marginpar{make sure we understand this} 

Let $i_t$ be the arm queried at time $t \in \mathbb{N}$ by $\A$. We may bound the KL-Divergence between $\text{Sim}(\pi(\nu), \Omega_t)$ and $\text{Sim}(\pi(\nu'), \Omega_t)$ as 
\begin{eqnarray*}
\max_{i_1, \cdots, i_T} \sum_{t=1}^T & & KL\left(\text{Sim}(\pi(\nu), \{i_s\}_{s=1}^t), \text{Sim}(\pi(\nu'), \{i_s\}_{s=1}^t\right) \\
& \leq & \tau KL(\pi(\nu)_{\pi(i^\ast)}, \pi(\nu')_{\pi(i^\ast)}) + \tau KL(\pi(\nu)_{\pi(k)}, \pi(\nu')_{\pi(k)}) \\
& = & \tau \frac{\beta^2}{2} + \tau \frac{\beta^2}{2}\\
& = & \tau \beta^2.
\end{eqnarray*}

By Lemma 1 of \cite{simchowitz2017simulator}, averaging over all permutations is equivalent to an algorithm first uniformly permuting the given instance and then undoing this before returning its answer. For any instance $\eta$, such an algorithm is symmetric in that
$$\P_\eta((i_1, \cdots, i_T) = (I_1, \cdots, I_T)) = \P_{\pi(\eta)}((\pi(i_1), \cdots, \pi(i_T)) = (\pi(I_1), \cdots, \pi(I_T))).$$

Namely, the probability that a given sequence of arms is sampled on $\eta$ is the same as the permutation applied to that sequence on $\pi(\eta)$. We assume that $\A$ is symmetric. Otherwise, we may use $\A$ to construct a symmetric algorithm by first permuting an instance before passing it to $\A$ and then permuting the output back. 

Since $W_{\pi(k)}(\Omega_t)$ and $W_{\pi(i^\ast)}(\Omega_t)$ are truthful on $\text{Sim}(\pi(\nu), \Omega_t)$ and $\text{Sim}(\pi(\nu'), \Omega_t)$ respectively, by Lemma~2 of \cite{simchowitz2017simulator}, we have that 
\begin{align*}
    \P_{\A, \pi(\nu)} &(W_{\pi(k)}(\Omega_t)) + \P_{\A, \pi(\nu')}(W_{\pi(i^\ast)}(\Omega_t)) \\ & \geq TV(\P_{\A, \pi(\nu)}, \P_{\A , \pi(\nu')}) - Q\left(KL(\text{Sim}(\pi(\nu), \Omega_t), \text{Sim}(\pi(\nu'), \Omega_t))\right)
\end{align*}
for $Q(\beta) = \min\{1 - 1/2e^{-\beta}, \sqrt{\beta/2}\}$. Since $\A$ is symmetric, for any permutation $\pi$, we have that
$$\P_{\A, \pi(\nu)}(W_{\pi(k)}(\Omega_t)) + \P_{\A, \pi(\nu')}(W_{\pi(i^\ast)}(\Omega_t)) = \P_{\A, \nu}(W_{k}(\Omega_t)) + \P_{\A, \nu'}(W_{i^\ast}(\Omega_t)) = 2\P_{\A, \nu}(W_{k}(\Omega_t))$$

Combining the above with the previous bounds on the total variation and KL divergence, we have that 

\begin{eqnarray*}
\P_{\A \times\nu}(N_k > \tau) = \P_{\A \times\nu}(W_k(\Omega_t)) \geq
\frac{1}{2}\left(1 - 2\delta  - \sqrt{\frac{\tau \beta^2}{2}}\right)
\end{eqnarray*}
Plugging in $\tau  = 1/2 \beta^2$, we see that $\P_{\A \times\nu}(N_k > 1/2 \beta^2) \geq 1/2(1/2 - 2\delta)$. Since $k$ was arbitrary, we may repeat this argument for each $k$ in $[n] \backslash \{i^\ast\}$. Combining this with Markov's inequality, we see that 

\begin{eqnarray*}
\E_{\A \times \nu} \left[\sum_{k \neq i^\ast}N_k \right] & \geq & \frac{1}{4}(1/2 - 2\delta) \sum_{k \neq i^\ast}\frac{1}{\beta^2} \\
& > & \frac{1}{16} \sum_{k \neq i^\ast}\frac{1}{\beta^2} \\
& = & \frac{1}{16}\frac{n-1}{\beta^2}
\end{eqnarray*}
where the final inequality follows from $\delta < 1/16$. The above holds for any $\delta$-PAC algorithm $\A$. 
\end{proof}

\begin{theorem}\label{thm:1spike_complexity}
Fix $n$ and $\beta$ and consider a set $\nu$ of $n$ Gaussian random variables such that for a uniformly random chosen $i^\ast \in [n]$, $\rho_{i^\ast} = {\cal N}(\beta, 1)$. Fix $\delta < 1/16$ and a uniformly sampled permutation $\pi$.
Any $\delta$-PAC algorithm to detect $i^\ast$ on $\nu$ requires
$$\frac{1}{16}\frac{n-1}{\beta^2} + \frac{2}{\beta^2}\log(1/2.4\delta)$$
samples in expectation, where the expectation is taken both over the randomness in the permutation, the randomness in $\pi(\nu)$, and any internal randomness to the algorithm. 
\end{theorem}

\begin{proof}
By Lemma~\ref{lem:1spike_kauf}, arm $i^\ast$ must be sampled $\frac{2}{\beta^2}\log(1/2.4\delta)$ times. By Theorem~\ref{thm:simulator}, arms in $[n]\backslash \{i^\ast\}$ must collectively be sampled $\frac{1}{16}\frac{n-1}{\beta^2}$ times. Joining these two results 
gives the stated result. 
\end{proof}

\subsection{Hypothesis testing lower bounds}\label{sec:hypo_test}
Next, we consider a binary hypothesis test that is related to the question of $1$-spike detection. As we will show, this test has the interesting property that the alternate hypothesis may be declared in $O(n)$ fewer samples than the null. In particular, this observation allows us to significantly sharpen the result of Theorem 3.1 of \cite{castro2014adaptive} in the case that the alternate hypothesis is true. 

\begin{definition}[$\beta$-Single Spike Hypothesis Test]
Consider an instance $\nu = \{\rho_1, \cdots, \rho_n\}$ of $n$ unit variance Gaussian distributions. By sampling individual distributions $\rho_i$, one wishes to perform the following test:

\textbf{Null Hypothesis $H_0$:} $\rho_i = {\cal N}(0,1)$ for all $i \in [n]$. 

\textbf{Alternate Hypothesis $H_1$:} the instance $\nu$ is drawn uniformly from the set $\{\nu_i: \rho_i = {\cal N}(\beta,1), \rho_j = {\cal N}(0,1) \ \forall \ j \neq i\}$. 
\end{definition}

For any instance $\nu$, we say ``$H_1$ is true on $\nu$'' if $\exists i: \rho_i = {\cal N}(\beta, 1)$ and otherwise we say ``$H_0$ is true on $\nu$.''
Next, we bound the sample complexity of any algorithm to perform the $\beta$-Single Spike Hypothesis Test with probability at least $1-\delta$ in the case that $H_0$ is true. 

\begin{lemma}\label{lem:H0_low}
Fix $n$, $\beta$, and $\delta$ and consider a set $\nu$ of $n$ standard normal random variables where $H_0$ is true. Any algorithm to correctly declare $H_0$ in the $\beta$-Single Spike Hypothesis Testing problem with probability at least $1-\delta$ requires
$$\frac{2n}{\beta^2}\log\left(\frac{1}{2.4\delta}\right) $$
samples in expectation.
\end{lemma}

\begin{remark}
This matches the worst case result of Theorem~3.1 in \cite{castro2014adaptive}. However, as we will show in the following theorem, when $H_1$ is true, this can be significantly improved. 
\end{remark}

\begin{proof}
Notice that for each $i \in [n]$, we may construct an alternate instance $\nu_i$ by changing the distribution of $\rho_i$ to be ${\cal N}(\beta, 1)$ and leaving others unchanged. On $\nu_i$, $H_1$ is instead true. To distinguish between $\nu$ and $\nu_i$, necessary to declare $H_0$ versus $H_1$, by Lemma 1 of \cite{kaufmann2016complexity}, any $\delta$-PAC algorithm requires $\E_\nu[N_i] \geq \frac{2}{\beta^2}\log(1/2.4\delta)$ where $\E_\nu$ denotes expectation with respect to the instance $\nu$ and $N_i$ denotes the number of samples of arm $i$. Repeating this argument for each $i \in [n]$ gives the desired result. 
\end{proof}

To lower bound the expected sample complexity of any algorithm to perform the $\beta$-Single Spike Hypothesis Test in the setting where $H_1$ is true, we consider a reduction to the $1$-spike detection problem studied in \ref{sec:1spike_detect}. In particular, we show that $O(n\beta^{-2} + \beta^{-2}\log(1/\delta))$ samples are necessary to perform this test. Hence, for small $\delta$, this rate is $O(n)$ faster than the the lower bound in Lemma~\ref{lem:H0_low}. 
For the reduction to $1$-spike detection, we show that if there is an algorithm to declare $H_1$ in fewer than $O(n\beta^{-2})$ samples, then one can design an algorithm akin to binary search for the $1$-spike detection problem that returns $i^\ast$ in fewer than $O(n\beta^{-2})$ samples, contradicting Lemma~\ref{thm:simulator}. 

\begin{lemma}\label{lem:H1_low}
Fix $n$, $\beta$, and $\delta < 1/16$. Let $\pi$ be a random permutation. Consider an instance $\nu$ where $H_1$ is true. In this setting, any algorithm to correctly declare $H_1$ in the $\beta$-Single Spike Hypothesis Testing problem on $\pi(\nu)$ with probability at least $1-\delta$ requires
$\frac{1}{32}\frac{n}{\beta^2}$
samples in expectation.
\end{lemma}

\begin{proof}
Fix $\delta > 0$ and let $i^\ast$ denote the single ``spike'' distribution such that $\rho_{i^\ast} = {\cal N}(\beta,1)$. 
Assume for contradiction that there is an algorithm $\A(\pi(\nu), \delta, \beta)$ that correctly declares $H_1$ on $\pi(\nu)$ in at most $\frac{1}{32}n\beta^{-2}$ samples in expectation with probability at least $1-\delta$ on any instance $\pi(\nu)$ of $n$ distributions if $H_1$ is true. Otherwise, if $H_0$ is true, assume that $\A$ correctly declares $H_0$ in an arbitrary number of samples lower bounded by Lemma~\ref{lem:H0_low}. As in the proof of Theorem~\ref{thm:simulator}, we may assume that $\A$ is symmetric in that its expected sample complexity is independent of $\pi$ and therefore drop the dependence on $\pi$ for the remainder of the proof.
For simplicity, assume that $n = 2^k$ for some $k \in \N$. Otherwise, we may hallucinate $2^{\lceil \log_2(n)\rceil} - n$ standard normal distributions and form an instance $\nu'$ comprised of these additional distribution and those in $\nu$. If so, anytime $\A$ requests a sample from a distribution in $\nu' \backslash \nu$, draw a sample from ${\cal N}(0,1)$ and pass it to $\A$, only tracking the number of samples drawn from $\nu$. 

% \textbf{Step $0$: A method to declare $H_0$}
% First, we develop a method to declare $H_0$ for $\beta$-single spike hypothesis testing. Consider the following uniform sample procedure.

% \begin{algorithm}[H]
% \caption{\texttt{Uniform}: An algorithm for $\beta$-single spike hypothesis testing}
% \begin{algorithmic}[1]
% \Require{$\delta > 0$, $\beta > 0$, instance $\nu$}
% \State{Let $\hat{\mu}_i$ denote the empirical mean of the $i^\text{th}$ distribution}
% \For{$t = 1, \cdots, \lceil 4\beta^{-2}\log(2n/\delta)\rceil$}
% \For{$i = 1, \cdots, n$}
%     \State{Pull arm $i$ and update $\hat{\mu}_i$}
% \EndFor
% \EndFor
% \If{$\exists i: \hat{\mu}_i > \beta/2$}
% \State{Declare $H_1$}
% \Else
% \State{Declare $H_0$}
% \EndIf
% \end{algorithmic}
% \end{algorithm}

% By Hoeffding's inequality and a union bound over the $n$ distributions in $\nu$,
% $$\P \left(\bigcup_{i=1}^n |\mu_i - \hat{\mu}_i| > \beta/2\right) \leq \delta.
% $$
% Therefore, with probability at least $1-\delta$, $\exists i: \hat{\mu}_i > \beta/2$ if and only if $H_1$ is true. Hence, the above method correctly performs the $\beta$-single spike hypothesis test with probability at least $1-\delta$. Summing over the $n$ distributions, this method draws exactly $\lceil 4n\beta^{-2}\log(2n/\delta)\rceil$ samples. Note that this is optimal up to a $\log(n)$ factor by Lemma~\ref{lem:H0_low}. 
% Next, we use the above routine and the assumed algorithm $\A$ to develop a method to perform $1$-Spike detection on $\nu$. 
In what follows, we use $\A$ to develop a method for $1$-Spike detection. To do so, we show that one may use $\A$ to perform binary search for the distribution $i^\ast$ such that $\rho_{i^\ast} = {\cal N}(\beta, 1)$ and this leads to a contradiction of Theorem~\ref{thm:simulator}. For ease of exposition, for $i <j$, let $\nu[i:j] := \{\rho_i, \cdots, \rho_j \}$, the subset of instance $\nu$ with distributions $i, \cdots, j$. If $H_1$ is true on $\nu[i:j]$, by assumption, with probability at least $1 - \delta$,
$\A$ correctly declares $H_1$ on $\nu[i:j]$ in at most $\frac{1}{32}(j-i + 1)\beta^{-2}$ samples in expectation. 

\begin{algorithm}[H]
\caption{An algorithm for $1$-spike detection \label{alg:1spike_alg}}
\begin{algorithmic}[1]
\Require{$\delta > 0$, $\beta > 0$, instance $\nu$ such that $H_1$ is true, algorithm $\A$}
\State{Let $\text{Low} = 1$ and $\text{High} = n$}
\For{$i = 1, \cdots, \log_2(n)$}
\State{1) Let $\text{Mid} = 1 + (\text{Low} + \text{High})/2$}
\State{2) In parallel, run $\A_{\text{Low}} = \A(\nu[\text{Low}:\text{Mid}-1], \beta, \delta/2\log_2(n))$ and $\A_{\text{High}} =\A(\nu[\text{Mid}: \text{High}], \beta, \delta/2\log_2(n))$}
\State{3) If either routine declares $H_1$, terminate the other}
\If{$\A_{\text{Low}}$ declares $H_1$}
    \State{$\text{High} = \text{Mid}-1$}
\Else 
    \State{$\text{Low} = \text{Mid}$ \vspace{0.3em}}
\EndIf 
\EndFor
\Return{$\text{Low}$}
\end{algorithmic}
\end{algorithm}

In step 2) if the loop, we separately run
$\A$ in parallel on $\nu[\text{Low}:\text{Mid}-1]$ and $\nu[\text{Mid}:\text{High}]$, each with failure probability $\delta/2\log(n)$. We alternate between passing a sample to $\A_{\text{Low}}$ and to $\A_{\text{High}}$. In Step 3), we terminate $\A_{\text{High}}$ if $\A_{\text{Low}}$ declares $H_1$ and vice versa. This process continues until $\text{High} = \text{Low}$, when there is a single distribution remaining and the algorithm declares it as the spike with mean $\beta$. 


First, we show that this algorithm is correct with probability at least $1-\delta$. The algorithm errs if and only if in any round $i$, either $\A_\text{Low}$ or $\A_\text{High}$ errs each with occurs with probability at most $\delta/2\log_2(n)$. Union bounding over the $\log_2(n)$ rounds, we see that the algorithm errs with probability at most $1-\delta$. For the remainder of the proof, we will assume that in no round does either $\A_\text{Low}$ or $\A_\text{High}$ incorrectly declare $H_0$ or $H_1$ if the reverse is true.

Next, we bound the expected total number of samples drawn by the algorithm. Let $T$ denote the random variable of the total number of samples Algorithm~\ref{alg:1spike_alg} draws when run on instance $\nu$. Let $T^i$ denote the number of samples drawn in round $i$. 
% Recall that the expected sample complexity of $\A$ on $\nu[i:j]$ is at most $(j - i + 1)\beta^{-2}$ by assumption. To differentiate between $\A_\text{Low}$ and $\A_\text{High}$ in different rounds, we denote $\A_\text{Low}^i$ and $\A_\text{High}^i$ as $\A_\text{Low}$ and $\A_\text{High}$ in round $i$. 
Therefore, we may write
$$\E_\nu [T] =\sum_{i=1}^{\log_2(n)} \E_\nu[T^i].$$
Next, we bound $\E_\nu[T^i]$. The number of distributions sampled in round $i$ is $n/2^i$ deterministically and samples are not shared across rounds. Therefore, the $T^i$'s are independent. As we have assumed the high probability event that $\A_\text{Low}$ and $\A_\text{High}$ do not err in any round, $i^\ast$ is not removed. Therefore in any round $i$, $H_1$ is true for either $\nu[\text{Low}:\text{Mid}-1]$ or $\nu[\text{Mid}: \text{High}]$. Therefore, either $\A_\text{Low}$ or $\A_\text{High}$ terminates in at most $\frac{n}{32 \cdot 2^i\beta^2}$ samples in expectation. In Step 3) of the algorithm, we terminate $\A_\text{High}$ if $\A_\text{Low}$ declares $H_1$ and vice versa. Hence, $\E_\nu[T^i] \leq \frac{n}{16 \cdot 2^i\beta^2} $. Therefore, 
\begin{align*}
    \E_\nu [T] \leq \sum_{i=1}^{\log_2(n)} \frac{n}{16 \cdot 2^i\beta^2} = \frac{1}{16}\frac{n-1}{\beta^2}
\end{align*}
However, this contradicts Theorem~\ref{thm:simulator} for $\delta < 1/16$. Hence no such algorithm $\A$ exists and any algorithm to declare $H_1$ on instance $\nu$ requires at least $\frac{1}{32}\frac{n}{\beta^2}$ samples in expectation.
\end{proof}

\begin{theorem}\label{thm:beta_hypo_test}
Fix $n$, $\beta$, and $\delta < 1/16$ and consider an instance $\nu$. If $H_0$ is true on $\nu$, any algorithm requires at least 
$$\frac{2n}{\beta^2}\log\left(\frac{1}{2.4\delta}\right) $$
samples in expectation to perform the $\beta$-Single Spike Hypothesis Test. If $H_1$ is true on $\nu$, any algorithm requires at least 
$$\frac{1}{64}\frac{n}{\beta^2} + \frac{1}{\beta^2}\log\left(\frac{1}{2.4\delta}\right) $$
samples in expectation to perform the $\beta$-Single Spike Hypothesis Test.
\end{theorem}

\begin{remark}
This matches the worst case result of Theorem 3.1 of \cite{castro2014adaptive}. However, this highlights that if $H_1$ is true, that result can be sharpened by a factor of $O(n)$ for small $\delta$. 
\end{remark}

\begin{proof}
If $H_0$ is true for $\nu$, the result follows immediately from Lemma~\ref{lem:H0_low}.
Otherwise, assume $H_1$ is true for $\nu$ and let $i^\ast$ be the single distribution such that $\rho_{i^\ast} = {\cal N}(\beta, 1)$. Similar to the proof of Lemma~\ref{lem:1spike_kauf}, one may consider an alternate instance $\nu'$ where $\rho_{i^\ast} = {\cal N}(0, 1)$ and all other distributions are unchanged. Therefore, on $\nu'$, $H_0$ is true and any algorithm that is correct with probability at least $1-\delta$ must be able to distinguish between these two instances.
By Lemma 1 of \cite{kaufmann2016complexity}, any algorithm that is correct with probability at least $1-\delta$ must therefore sample $i^\ast$ $\frac{2}{\beta^2}\log\left(\frac{1}{2.4\delta}\right)$ times. Combining this with the result of Lemma~\ref{lem:H1_low}, any algorithm that is correct with probability at least $1-\delta$ must collect at least 
$$\max\left\{\frac{1}{32}\frac{n}{\beta^2},  \frac{2}{\beta^2}\log\left(\frac{1}{2.4\delta}\right)\right\} \geq \frac{1}{64}\frac{n}{\beta^2} + \frac{1}{\beta^2}\log\left(\frac{1}{2.4\delta}\right)$$
samples in expectation. 
\end{proof}

\subsection{Moderate confidence bounds for finding All $\epsilon$-good arms}
In this setting, we prove that there is an instance such that any algorithm to return all $\epsilon$-good arm must also draw at least $O(n\beta^{-2})$ samples in expectation, and this allows us to develop a sharper lower bound than the one presented in Theorem~\ref{thm:inst_lower}. To do so, we prove a reduction from finding all $\epsilon$-good arms to the $\beta$-single spike hypothesis test. In particular, we show that if one has a generic method to find all $\epsilon$-good arms (with slack $\gamma=0$), then one may use this to develop a method to perform the $\beta$-single spike hypothesis test. Therefore, lower bounds on the this test apply to the problem of finding all $\epsilon$-good arms as well. 

\begin{lemma}\label{lem:beta_reduction}
Fix $n > 200$, $\epsilon > 0$, $0 < \beta < \epsilon/2 $, and $\delta < 1/32$.
Let $\nu$ be an instance such that $\mu_1 = 2\beta$, $\mu_2 = \cdots = \mu_{n-1} = 0$, and $\mu_n = \beta - \epsilon$. Select a permutation $\pi:[n] \rightarrow [n]$ uniformly from the set of $n!$ permutations, and consider the permuted instance $\pi(\nu)$. Any algorithm that returns $G_\epsilon(\pi(\nu))$ on $\pi(\nu)$ with correctly probability at least $1-\delta$ requires at least 
$c_7\frac{n}{\beta^2}$
samples in expectation for a universal constant $c_7$ where the expectation is taken jointly over the randomness in $\nu$ and $\pi$.
\end{lemma}

\begin{proof}
Assume that there exists a generic algorithm $\A(v, \epsilon, \delta)$ that returns a set $G$ such that $G = G_\epsilon(v)$ with probability at least $1-\delta$ for any instance $v$. By Lemma 1 of \cite{simchowitz2017simulator}, averaging over all permutations is equivalent to first permuting the instance $v$ and then passing it to $\A$ and undoing the permutation when returning the answer. We therefore assume that $\A$ is \emph{symmetric} in that
its expected sample complexity of $\A$ is invariant to the permutation $\pi$. Otherwise, we may use $\A$ to form a symmetric algorithm.
%by permuting its inputs, running $\A$, and then undoing the permutation on the output. 


% upon which one wishes to perform $2\beta$-single spike hypothesis test. Recall that under $H_0$, $\mu_{\pi(i)} = 0$ for all $\rho_{\pi(i)} \in \pi(\nu)$ and under $H_1$, there exists an $i^\ast$ such that $\mu_{\pi(i^\ast)} = 2\beta$ and $\mu_{\pi(i)} = 0$ for all $\pi(i) \neq \pi(i^\ast)$.

% \textbf{Step 0 - reducing all-$\epsilon$ to $2\beta$-single spike hypothesis testing:}
To prove this Lemma, we will consider a reduction to the $2\beta$-single spike hypothesis test (as opposed to $\beta$ in Section \ref{sec:hypo_test}). 
To do so, consider a second instance $\nu'$ such that $\mu_1 \in \{0, 2\beta\}$ (chosen randomly) and $\mu_2 = \cdots \mu_n = 0$. Suppose one wishes to perform the $2\beta$-single spike hypothesis on $\pi(\nu')$. Recall that if $H_0$ is true, then $\mu_i = 0$ for all $i \in [n]$, hence $\mu_1 = 0$. 
Otherwise, if $H_1$ is true, $\mu_1 = 2\beta$. 
% We proceed by showing a reduction from the problem of finding all $\epsilon$-good arms on $\pi(\nu)$ to performing the $2\beta$-single spike hypothesis test on $\pi(\nu')$. 
Consider the following procedure that uses $\A$ to perform the hypothesis test:

\begin{algorithm}[H]
\caption{Using All-$\epsilon$ for $2\beta$-single spike hypothesis testing \label{alg:all_eps_hypotest}}
\begin{algorithmic}[1]
\Require{$\delta > 0$, $\epsilon > 0$, $0 < \beta < \epsilon/2$, instance $\pi(\nu)$ such that $H_1$ is true, and algorithm $\A$}
% \State{\textbf{Step 1:} Apply permutation $\pi$ to $\nu'$}
\State{\textbf{Step 1:} Choose an index $\hat{i} \in [n]$ uniformly}
\State{\textbf{Step 2:} Sample arm $\hat{i}$ $\left\lceil\beta^{-2}\log(2/\delta) \right\rceil$ and compute empirical mean $\hat{\mu}_{\hat{i}}$}
\If{$\hat{\mu}_{\hat{i}} > \beta$}
    \State{Declare $H_1$ and terminate}
\EndIf
\State{\textbf{Step 3:} Let $\nu''$ be the instance $$ \nu'' = \begin{cases}
\rho_{\pi(i)} & \text{ if } \pi(i) \neq \hat{i}\\
\rho_{\pi(i)} -\epsilon + \beta & \text{ if } \pi(i) = \hat{i}
\end{cases}$$}
% \State{\textbf{Step 4:} 
% Replace $ \rho_{\hat{i}} $ with $\rho_{\hat{i}} - \epsilon + \beta$ in instance $\pi(\nu')$}
\State{\textbf{Step 4:} $G = \A(\pi(\nu''), \epsilon, \delta)$}
\If{$\hat{i} \in G$}:
\State{Declare $H_0$ and terminate}
\Else
\State{Declare $H_1$ and terminate}
\EndIf
\end{algorithmic}
\end{algorithm}

First, by Hoeffding's inequality,
$\P(|\mu_{j} - \hat{\mu}_{j}| > \beta | \hat{i} = j) \leq \delta$. Therefore, 
$$\P(|\mu_{\hat{i}} - \hat{\mu}_{\hat{i}}| > \beta |) = \sum_{j=1}^n\P(|\mu_{j} - \hat{\mu}_{j}| > \beta | \hat{i} = j)\P(\hat{i} = j) \leq \delta \sum_{j=1}^n\P(\hat{i} = j) = \delta.$$
Hence, if $\hat{\mu}_{\hat{i}} > \beta$, then $\mu_{\hat{i}} > \beta$ with probability at least $1-\delta$ and the method correctly declares $H_1$. This step ensures that the selected arm $\hat{i}$ is not distributed ${\cal N}(2\beta, 1)$ in the case that $H_1$ is true on $\pi(\nu')$. 
% Furthermore, on $H_1$, this implies that $\hat{i} \neq \pi(1)$. 

Otherwise, the method replaces $\rho_{\hat{i}}$ with $\rho_{\hat{i}} - \epsilon + \beta$ such that $\hat{\mu}_{\hat{i}} = \beta - \epsilon$
and runs $\A$ on this new instance $\nu''$. If $H_0$ is true on $\pi(\nu')$, all other distributions have mean $0$, and $\hat{i}$ therefore is $\epsilon$-good on instance $\nu''$. If $H_1$ is true on $\pi(\nu')$, then $\rho_{\pi(1)} = {\cal N}(2\beta, 1)$ and $\hat{i}$ is not $\epsilon$-good on instance $\nu''$. Since $\A$ is run with failure probability $\delta$, this test is correct with probability at least $1-2\delta$. 

Let $\T_{\A}(\pi(\nu''))$ denote the random variable of the number of samples drawn by $\A$ on instance $\pi(\nu'')$ and let $T$ denote the random variable of the total number of samples drawn by this procedure. Therefore, 
$\E[T] \leq \E[\T_{\A}(\pi(\nu''))] + \left\lceil\beta^{-2}\log(2/\delta) \right\rceil$. 

If $H_1$ is true on $\nu'$, then $\nu''$ is equal to $\nu$ up to a permutation. Since we have assumed that $\A$ is symmetric, $\E[\T_{\A}(\pi(\nu''))] = \E[\T_{\A}(\pi(\nu))] = \E[\T_{\A}(\nu)]$. Hence, $\E[T] \leq \E[\T_{\A}(\nu)] + \left\lceil\beta^{-2}\log(2/\delta) \right\rceil$ if $H_1$ is true on $\nu'$. However, by Theorem~\ref{thm:beta_hypo_test}, if $H_1$ is true, 
$$\E[T] \geq \frac{1}{256}\frac{n}{\beta^2} + \frac{1}{4\beta^2}\log\left(\frac{1}{4.8\delta}\right).$$
Combining this with the previous, 
$$\E[\T_{\A}(\nu)] + \left\lceil\beta^{-2}\log(2/\delta) \right\rceil \geq \frac{1}{256}\frac{n}{\beta^2} + \frac{1}{\beta^2}\log\left(\frac{1}{4.8\delta}\right). $$
Therefore, for $n > 200$ 
$$ 4\E[\T_{\A}(\nu)]+4 \geq \frac{n}{\beta^2}\left(\frac{1}{64} - \frac{\log(4.8)}{n} \right) > \frac{1}{128} \frac{n}{\beta^2}.$$
Hence, for a constant $c_2$, $\E[\T_{\A}(\nu)] \geq c_2 \frac{n}{\beta^2}$. Therefore, any algorithm $\A$ that is correct with probability at least $1-\delta$ requires at least $c_2 \frac{n}{\beta^2}$ samples on instance $\nu$. 
\end{proof}

With the above proof, we restate the following minimax lower bound on the sample complexity of returning all $\epsilon$-good stated in Section~\ref{sec:lower_bound}. In particular, this bound highlights \emph{moderate confidence} terms that are independent of $\delta$. Moderate confidence terms have been studied in works such as \cite{simchowitz2017simulator, chen2017nearly}. Despite being independent of $\delta$, these terms can have important effects in real world scenarios. The following bound demonstrates that there are instances for which moderate confidence terms are necessary for finding all $\epsilon$-good arms. Moderate confidence terms likewise appear in the upper bound of the complexity of \texttt{FAREAST}, Theorem~\ref{thm:fareast_complex}.

\begin{theorem}
Fix $n > 200$, $\epsilon > 0$, $\beta < \epsilon/16$, and $\delta < 1/32$.
Let $\nu$ be an instance of $n$ Gaussian distributions such that $\mu_1 = \epsilon$, $\mu_2 = \cdots = \mu_{n-1} = \epsilon - 2\beta$, and $\mu_n = -\beta$ and each have variance $1$. 
% Let $\nu$ be an instance such that $\mu_1 = 2\beta$, $\mu_2 = \cdots = \mu_{n-1} = 0$, and $\mu_n = \beta - \epsilon$. 
Select a permutation $\pi:[n] \rightarrow [n]$ uniformly from the set of $n!$ permutations, and consider the permuted instance $\pi(\nu)$. Any algorithm that returns $G_\epsilon(\pi(\nu))$ on $\pi(\nu)$ with correctly probability at least $1-\delta$ requires at least 
$$c_2\frac{n}{\beta^2} + c_2\left( \frac{n-1}{\epsilon^2} +\frac{1}{\beta^2}\right)\log \left(\frac{1}{2.4\delta}\right)$$ 
samples in expectation over the randomness in $\nu$ and $\pi$ for a universal constant $c_2$.
\end{theorem}

\begin{remark}
For the same instance, Theorem~\ref{thm:inst_lower} would imply a lower bound of 
$$O\left(\left( \frac{n-1}{\epsilon^2} +\frac{1}{\beta^2}\right)\log \left(\frac{1}{2.4\delta}\right)\right)$$ 
\end{remark}

\begin{proof}
We may equivalently consider the same instance with all means shifted down by $\epsilon - 2\beta$ since a method for that instance could be used to return all $\epsilon$ good arms in the stated instance. 
By Lemma~\ref{lem:beta_reduction}, $c_2\frac{n}{\beta^2}$ samples are necessary in expectation. 
By Theorem~\ref{thm:inst_lower}, 
$$\frac{1}{16}\sum_{i=1}^n \max \left(\frac{1}{\left(\epsilon - \Delta_i \right)^{2}}, \min \left\{\frac{1}{\Delta_i^2}, \frac{1}{\alpha^2}\right\} \right) \log \left(\frac{1}{2.4\delta}\right)$$
samples are necessary in expectation. For $\pi(1)$, 
$$\max \left(\frac{1}{\left(\epsilon - \Delta_i \right)^{2}}, \min \left\{\frac{1}{\Delta_i^2}, \frac{1}{\alpha^2}\right\} \right) = \max \left(\frac{1}{\epsilon^{2}}, \frac{1}{(\epsilon - 2\beta)^2} \right) = \frac{1}{(\epsilon - 2\beta)^2}$$
For $\pi(n)$
$$\max \left(\frac{1}{\left(\epsilon - \Delta_i \right)^{2}}, \min \left\{\frac{1}{\Delta_i^2}, \frac{1}{\alpha^2}\right\} \right) = \frac{1}{\beta^{2}}$$
Otherwise, since $\beta < \epsilon/16$
$$\max \left(\frac{1}{\left(\epsilon - \Delta_i \right)^{2}}, \min \left\{\frac{1}{\Delta_i^2}, \frac{1}{\alpha^2}\right\} \right) = \max \left(\frac{1}{(\epsilon - 2\beta)^2}, \min \left\{\frac{1}{4\beta^2}, \frac{1}{(\epsilon - 2\beta)^2}\right\} \right) = \frac{1}{(\epsilon - 2\beta)^2}.$$
Therefore, 
$$\frac{1}{16}\left(\frac{n-1}{(\epsilon - 2\beta)^2} + \frac{1}{\beta^2}\right)\log \left(\frac{1}{2.4\delta}\right) \geq \frac{1}{16}\left(\frac{n-1}{\epsilon^2} + \frac{1}{\beta^2}\right)\log \left(\frac{1}{2.4\delta}\right) $$
samples are necessary in expectation. Since both this and $c_2\frac{n}{\beta^2}$ are valid lower bounds, the average is also a valid bound. 
Hence, any algorithm requires 
$$ \frac{c_2}{2}\frac{n}{\beta^2} + \frac{1}{32}\left(\frac{n-1}{\epsilon^2} + \frac{1}{\beta^2}\right)\log \left(\frac{1}{2.4\delta}\right)$$
samples in expectation, where the expectation is taken over the randomness in the instance $\nu$ and random permutation $\pi$. 
\end{proof}

==> mod_east_complex.tex <==
The proof proceeds in a manner similar to the proof of Theorem~\ref{thm:east_complexity}by first obtaining bounds on $T_i$. 
For arm~$i \in G_{\Gamma}^c$, we show $T_i \leq h(\Delta_i'/(2+2\mathcal{L}), \delta/n)$ by arguing that in the good event $\cE$, for all $t > h(\Delta_i'/(2+2\mathcal{L}), \delta/n)$ the arm~$i$ is not in $\A(t)$.
Let $j^\ast := \arg \max_{j \in \mathcal{A}(t)} \hat{\mu}_j$. Then, 
\begin{align*}
&\hat{\mu}_i + C_{\delta/n}(t) &&< L_{t} = \min_{x \in [\hat{\mu}_{j^\ast} - C_{\delta/n}(t), \hat{\mu}_{j^\ast} + C_{\delta/n}(t)]}\Gamma(x)\\
& && < \min_{x \in [\hat{\mu}_1 - C_{\delta/n}(t), \hat{\mu}_{j^\ast} + C_{\delta/n}(t)]}\Gamma(x),\\
&\overset{\cE}{\Leftarrow} \mu_i + 2C_{\delta/n}(t) &&< \min_{x \in [\mu_1 - 2C_{\delta/n}(t), \mu_{j^\ast} + 2C_{\delta/n}(t)]}\Gamma(x) 
< \min_{x \in [\mu_1 - 2C_{\delta/n}(t), \mu_1 + 2C_{\delta/n}(t)]}\Gamma(x)\\
& &&< \Gamma(\mu_1) - 2\mathcal{L}C_{\delta/n}(t),\\
& \Leftrightarrow (2+2\mathcal{L})C_{\delta/n}(t) && < \Gamma(\mu_1) - \mu_i =: \Delta_i' \Leftarrow t \geq  h(\Delta_i'/(2 + 2\mathcal{L}), \delta/n).
\end{align*}
The chain of inequalities above are true as we are increasing the domain of the minimization at each step. The reverse implication is true under $\cE$. We can argue about $T_i$ for $i \in G_\Gamma$ in a similar manner. Furthermore, for $i \in G_\Gamma, T'_i \leq h(0.25\Delta_i, \delta/n)$ is true in exactly the same way as before.
To obtain the final sample complexity, we use $T_\beta$ and $T_\gamma$. As before, $T_\beta = \max_i\{T_i\} = h(\min(\alpha_\epsilon', \beta_\epsilon')/(2+2\mathcal{L}), \delta/n)$. The only difference is in the expression for $T_\gamma$, which because of the stopping condition in modified \texttt{EAST}, is defined as 
\begin{equation*}
T_\gamma := \min \{t: \max(2C_{\delta/n}(t), U_t - L_t) \leq \gamma/2\}.
\end{equation*}
$2C_{\delta/n}(t) \leq \gamma/2$ is ensured when $t > h(0.25\gamma, \delta/n)$. For the other part, we have that
\begin{align*}
U_t - L_t = \max_{x \in [\hat{\mu}_{j^\ast} - C_{\delta/n}(t), \hat{\mu}_{j^\ast} + C_{\delta/n}(t)]}\Gamma(x)
- 
\min_{x \in [\hat{\mu}_{j^\ast} - C_{\delta/n}(t), \hat{\mu}_{j^\ast} + C_{\delta/n}(t)]}\Gamma(x)
\leq 2\mathcal{L}C_{\delta/n}(t).
% \\
% &\leq \max_{x \in [\hat{\mu}_{1} - C_{\delta/n}(t), \hat{\mu}_{j^\ast} + C_{\delta/n}(t)]}\Gamma(x)
% - 
% \min_{x \in [\hat{\mu}_{1} - C_{\delta/n}(t), \hat{\mu}_{j^\ast} + C_{\delta/n}(t)]}\Gamma(x)\\
% &\overset{\cE}{\leq} \max_{x \in [\hat{\mu}_{1} - 2C_{\delta/n}(t), \hat{\mu}_{1} + 2C_{\delta/n}(t)]}\Gamma(x)
% - 
% \min_{x \in [\hat{\mu}_{1} - 2C_{\delta/n}(t), \hat{\mu}_{1} + 2C_{\delta/n}(t)]}\Gamma(x) \leq 4\mathcal{L}C_{\delta/n}(t).
\end{align*}
Thus $U_t - L_t \leq \gamma/2$ is ensured when $2\mathcal{L}C_{\delta/n}(t) \leq \gamma/2$, which occurs when $t \geq h(0.25\gamma/\mathcal{L}, \delta/n)$. Thus $T_\gamma = h(0.25\gamma/\max(1,\mathcal{L}), \delta/n)$. Plugging in the expressions we obtain the final sample complexity as
\begin{align*}
\sum_{i=1}^n &  \min\left\{\max\left\{h\left(\frac{\Delta_i'}{2 + 2\mathcal{L}}, \frac{\delta}{n} \right), \min \left[h\left(0.25\Delta_i, \frac{\delta}{n} \right), h\left(\frac{1}{2+2\mathcal{L}}\min(\alpha_\epsilon', \beta_\epsilon'), \frac{\delta}{n} \right)\right] \right\},\right.\\
& \hspace{1cm}\left. h\left(\frac{0.25\gamma}{\max(1, \mathcal{L})}, \frac{\delta}{n} \right)\right\}
\end{align*}

Finally, we use Lemma~\ref{lem:inv_conf_bounds} to bound the function $h(\cdot, \cdot)$.
Since $\delta\leq 1/2$, $\delta/n \leq 2e^{-e/2}$. Further, recall that we have assumed $\max\{\frac{\Delta_i}{4}, \frac{\Delta_i'}{2+2\mathcal{L}}\} \leq 2$ for all $i$. Likewise, this implies that $\frac{\min{\alpha_\epsilon', \beta_\epsilon'}}{2+2\mathcal{L}} \leq 2$. 
Lastly, $\gamma \leq 8\max(1, \mathcal{L})$ implies that $\frac{0.25}{\max(1,\mathcal{L})} \leq 2$.
Therefore,
\begin{align*}
\sum_{i=1}^n &  \min\left\{\max\left\{h\left(\frac{\Delta_i'}{2 + 2\mathcal{L}}, \frac{\delta}{n} \right), \min \left[h\left(0.25\Delta_i, \frac{\delta}{n} \right), h\left(\frac{\min(\alpha_\epsilon', \beta_\epsilon')}{2+2\mathcal{L}}, \frac{\delta}{n} \right)\right] \right\},\right.\\
& \hspace{1cm}\left. h\left(\frac{0.25\gamma}{\max(1, \mathcal{L})}, \frac{\delta}{n} \right)\right\}\\
& \leq \sum_{i=1}^n\min\left\{\max\left\{\frac{8(1 + \mathcal{L})^2}{\Delta_i'^2}\log\left(\frac{2n}{\delta}\log_2\left(\frac{24(1+\mathcal{L}) n}{\delta\Delta_i'^2}\right) \right),\right.\right. \\
& \hspace{1cm}\left.\left.\min \left[\frac{64}{\Delta_i^2}\log\left(\frac{2n}{\delta}\log_2\left(\frac{192n}{\delta\Delta_i^2}\right) \right), \frac{8(1 + \mathcal{L})^2}{\min(\alpha_\epsilon', \beta_\epsilon')^2}\log\left(\frac{2n}{\delta}\log_2\left(\frac{24(1+\mathcal{L}) n}{\delta\min(\alpha_\epsilon', \beta_\epsilon')^2}\right) \right)\right] \right\},\right.\\
& \hspace{1cm}\left. \frac{64\max(1, \mathcal{L})}{\gamma^2}\log\left(\frac{2n}{\delta}\log_2\left(\frac{192\max(1, \mathcal{L})n}{\delta\gamma^2}\right) \right)
\right\}
\end{align*}
\qed 



% \subsection{Algorithm based on optimism}
% \input{NeurIPS_Submission/mod_ST2}

% \subsection{Sketch of proof of optimism algorithm}
% \textbf{The optimism algorithm}:
% \begin{itemize}
%     \item Let $\widehat{G}_\epsilon = \{i: \hat{\mu}_i > \max_j \hat{\mu}_j - \epsilon\}$, the set of empirically good arms
%     \item Let $U_t = \max_i u_i(t) - \epsilon$
%     \item Let $L_t = \max_j \ell_j(t) - \epsilon$ (note that a different arm can define $L_t$ and $U_t$)
% \end{itemize}
% At rounds until termination, we pull $3$ arms:
% \begin{enumerate}
%     \item $i^\ast(t) = \arg\max_i u_i(t)$
%     \item $i_1(t) = \arg\min_{i \in \widehat{G}_\epsilon}\ell_i(t)$
%     \item $i_2(t) = \arg\max_{i \in \widehat{G}_\epsilon^c} u_i(t)$
% \end{enumerate}
% Stop when for all arms $i$:
% $\text{either: } \ell_i(t) \geq U_t \text{ or } L_t \geq u_i(t)$, i.e., every arm is either declared as definitely good or definitely bad.


% \textbf{High level idea:} We decompose the event space as follows:

% I'll omit some log factors here and split things into claims. The idea is that if all claims are satisfied then we hit the stopping condition. 
% For brevity, let $\omega = \min(\alpha_\epsilon, \beta_\epsilon)$. Additionally, define the \emph{diameter} function for a set $S$: $D(S) = \max_{i, j \in S} u_i - \ell_i$, i.e., the largest confidence width within a set.

% % \begin{itemize}
% %     \item $i^\ast $ is not in $G_{\omega/2}$ (\textbf{Claim 1})
% %     \item $i^\ast $ is in $G_{\omega/2}$
% %     \begin{itemize}
% %         \item $i^\ast$ in $G_{\omega/2}$ and $D(G_{\omega/2}) > \omega/2$ (\textbf{Claim 2})
% %         \item $i^\ast$ in $G_{\omega/2}$ and $D(G_{\omega/2}) \leq \omega/2$
% %         \begin{itemize}
% %             \item ($i^\ast$ in $G_{\omega/2}$ and $D(G_{\omega/2}) \leq \omega/2$) and ($i_1 \in G_\epsilon^c$) (\textbf{Claim 3})
% %             \item ($i^\ast$ in $G_{\omega/2}$ and $D(G_{\omega/2}) \leq \omega/2$) and ($i_1 \in G_\epsilon$ and $\ell_{i_1}(t) < \mu_1 - \epsilon + \omega/2$) (\textbf{Claim 4})
% %             \item ($i^\ast$ in $G_{\omega/2}$ and $D(G_{\omega/2}) \leq \omega/2$) and ($i_2 \in G_\epsilon$) (\textbf{Claim 5})
% %             \item ($i^\ast$ in $G_{\omega/2}$ and $D(G_{\omega/2}) \leq \omega/2$) and ($i_2 \in G_\epsilon^c$ and $u_{i_2}(t) > \mu_1 - \epsilon - \omega/2$) (\textbf{Claim 6})
% %         \end{itemize}
% %     \end{itemize}
% % \end{itemize}
% \begin{itemize}
%     \item $i^\ast $ is not in $G_{\omega/2}$ (\textbf{Claim 1})
%     \item $i^\ast $ is in $G_{\omega/2}$ and:
%     \begin{itemize}
%         \item $D(G_{\omega/2}) > \omega/2$ (\textbf{Claim 2})
%         \item $D(G_{\omega/2}) \leq \omega/2$ and:
%         \begin{itemize}
%             \item $i_1 \in G_\epsilon^c$ (\textbf{Claim 3})
%             \item $i_1 \in G_\epsilon$ and $\ell_{i_1}(t) < \mu_1 - \epsilon + \omega/2$ (\textbf{Claim 4})
%             \item $i_2 \in G_\epsilon$ (\textbf{Claim 5})
%             \item $i_2 \in G_\epsilon^c$ and $u_{i_2}(t) > \mu_1 - \epsilon - \omega/2$ (\textbf{Claim 6})
%         \end{itemize}
%     \end{itemize}
% \end{itemize}

% \blake{Slight issue with how I was taking complements. Corrected below: }

% \begin{itemize}
%     \item $i^\ast $ is not in $G_{\omega/2}$ (\textbf{Claim 1})
%     \item $i^\ast $ is in $G_{\omega/2}$ and:
%     \begin{itemize}
%         \item $D(G_{\omega/2}) > \omega/2$ (\textbf{Claim 2})
%         \item $D(G_{\omega/2}) \leq \omega/2$ and:
%         \begin{itemize}
%             \item $i_1 \in G_\epsilon^c$ (\textbf{Claim 3})
%             \item $i_1 \in G_\epsilon$
%             and:
%             \begin{itemize}
%                 \item $i_2 \in G_\epsilon$ (\textbf{Claim 5:})
%                 \item $i_2 \in G_\epsilon^c$ (\textbf{See note below, Claim 4 and 6})
%             \end{itemize}
%         \end{itemize}
%     \end{itemize}
% \end{itemize}

% \textbf{Note - equivalent to step 4 (pg 19) of simulator draft:} All events assume conditions and true \emph{and} the algorithm has not terminated. When $i_1 \in G_\epsilon$ and $i_2 \in G_\epsilon^c$ and simultaneously, $D(G_{\omega/2}) \leq \omega/2$, this problem becomes thresholding with a fixed threshold. If we compare arms against $\mu_1 - \epsilon - \omega/2$ and $\mu_1 - \epsilon + \omega/2$, when the bounds separate from these fixed values, the alg must have terminated. 

% \textbf{Sketch of proof}

% \textbf{Claim 1:} $|\{t: i^\ast \notin G_{\omega/2}\}| \leq \sum_{i \in G_{\omega/2}^c}\frac{1}{\Delta_i^2}$

% \textbf{Proof idea:} Compare the upper bound of every arm in $G_{\omega/2}^c$ to $\mu_1$. Once it drops below, it can't be the highest UCB. 

% We have that $|\{t: i^\ast \notin G_{\omega/2}\}| = 
% \sum_{j \in G_{\omega/2}^c}
% |\{t: i^\ast(t)=j\}|$. We can bound the number of times an arm $j \in G_{\omega/2}^c$ can have the largest upper bound in the following manner.
% \begin{align*}
% |\{t: i^\ast(t) = j\}| &\overset{\cE}{=} 
% |\{t: i^\ast(t) = j \text{ and } u_j(t) \geq \mu_1\}| \\
% &\leq \max \{x: \hat{\mu}_j + C_{\delta/n}(x) \geq \mu_1\}\\
% &\overset{\cE}{\leq}
% \max \{x: \mu_j + 2C_{\delta/n}(x) \geq \mu_1\}
% = h(\Delta_j/2, \delta/n).
% \end{align*}
% Summing over all possible $j$ gives us the result.

% \textbf{Claim 2:} $|\{t: i^\ast \in G_{\omega/2} \text{ and }D(G_{\omega/2}) > \omega/2\}| \leq \sum_{i \in G_{\omega/2}}\frac{4}{\omega^2} = \sum_{i \in G_{\omega/2}}\frac{4}{\min(\alpha, \beta)^2} $

% \textbf{Proof idea:} Once every arm in the set gets $\sim 4\omega^{-2}$ pulls, all widths are less than $\omega/2$

% Let $T_j(t)$ denote the number of times arm~$j$ has been sampled up to time~$t$. 
% We have that $D_t(\{j\}) = u_j(t) - l_j(t) = 2C_{\delta/n}(T_j(t))$. This quantity is large only when $T_j(t)$ is small enough,
% $D_t(\{j\}) = 2C_{\delta/n}(T_j(t)) > \omega/4 \implies 
% T_j(t) < h(\omega/8, \delta/n)$.
% Under the good event $\cE$ all bounds are correct, and hence we have that 
% \begin{align*}
% D_t(G_{\omega/4}) = \max_{j, j' \in G_{\omega/4}} u_j(t) - \ell_{j'}(t) \leq 
% \mu_1 + \omega/8 - (\mu_1 - \omega/4 - \omega/8) = \omega/2.
% \end{align*}
% Since arm~$i^\ast(t)$ is sampled at each time~$t$, we get the required bound by summing over all $j \in G_{\omega/4}$. 

% \textbf{Claim 3:} $|\{t: i^\ast \in G_{\omega/2} \text{ and }D(G_{\omega/2}) \leq \omega/2 \text{ and } i_1 \in G_\epsilon^c\}| \leq \sum_{i\in G_\epsilon^c} \frac{1}{(\mu_i - (\mu_1 - \epsilon))^2}$

% \textbf{Proof idea:} Compare bad arms against a lower bound on the threshold. At some point the empirical mean cannot be above it. 

% Since $D(G_{\omega/4}) \leq \omega/2$, we have the following lower bound on the threshold value:
% $L^\ast(t) = \max_j \ell_{j}(t) - \epsilon \geq 
% \mu_1 - \omega/2 - \epsilon$. 
% For an arm $j \in G_{\epsilon}^c$, the number of times at which it can be the arm $i_1(t)$ can then be bounded as follows.
% \begin{align*}
% &|\{t: D_t(G_{\omega/4}) \leq \omega/2 \text{ and } i_1(t) = j\}|\\ 
% &= 
% |\{t: D_t(G_{\omega/4}) \leq \omega/2 \text{ and } i_1(t) = j \text{ and } L^\ast(t) \geq \mu_1 - \epsilon - \omega/2\}|\\
% &\leq \max \{x: \hat{\mu}_j + C_{\delta/n}(x) \geq \mu_1 - \epsilon - \omega/2\}\\
% &\leq \max \{x: \mu_j + 2C_{\delta/n}(x) \geq \mu_1 - \epsilon - \omega/2\} &&\text{(upper bound on LHS due to $\cE$)}\\
% &\leq \max \{x: 2C_{\delta/n}(x) \geq \mu_1 - \epsilon - \mu_j - \beta_\epsilon/2\} &&\text{(lower bound on RHS due to $\omega \leq \beta_\epsilon$)}\\
% &\leq \max \{x: 2C_{\delta/n}(x) \geq \mu_1 - \epsilon - \mu_j 
% - (\mu_1 - \epsilon - \mu_j)/2\} &&\text{(lower bound on RHS due to $\beta_\epsilon \leq \mu_1 - \epsilon - \mu_j$)}\\
% &= h((\mu_j - (\mu_1 - \epsilon))/4, \delta/n).
% \end{align*}
% Summing over all $j \in G_\epsilon^c$ gives us the bound.

% \textbf{Claim 4:} $|\{t: i^\ast \in G_{\omega/2} \text{ and }D(G_{\omega/2}) \leq \omega/2 \text{ and } i_1 \in G_\epsilon \text{ and } \ell_{i_1} < \mu_1 - \epsilon + \omega/2\}| \leq \sum_{i\in G_\epsilon} \frac{1}{(\mu_i - (\mu_1 - \epsilon))^2}$

% \textbf{Proof idea:} Compare $\ell_{i_1}$ to the fixed value $\mu_1 - \epsilon + \omega/2$

% \textbf{Claim 5:} $|\{t: i^\ast \in G_{\omega/2} \text{ and }D(G_{\omega/2}) \leq \omega/2 \text{ and } i_2 \in G_\epsilon\}| \leq \sum_{i\in G_\epsilon} \frac{1}{(\mu_i - (\mu_1 - \epsilon))^2}$

% \textbf{Proof idea:} Compare good arms against an upper bound on the threshold. At some point the empirical mean cannot be below it. 

% Since $D(G_{\omega/4}) \leq \omega/2$, we have the following upper bound on the threshold value:
% $U^\ast(t) = \max_j u_{j}(t) - \epsilon \leq 
% \mu_1 + \omega/2 - \epsilon$. 
% For an arm $j \in G_{\epsilon}$, the number of times at which it can be the arm $i_2(t)$ can then be bounded as follows.
% \begin{align*}
% &|\{t: D_t(G_{\omega/4}) \leq \omega/2 \text{ and } i_2(t) = j\}|\\ 
% &= 
% |\{t: D_t(G_{\omega/4}) \leq \omega/2 \text{ and } i_2(t) = j \text{ and } U^\ast(t) \leq \mu_1 - \epsilon + \omega/2\}|\\
% &\leq \max \{x: \hat{\mu}_j - C_{\delta/n}(x) \leq \mu_1 - \epsilon + \omega/2\}\\
% &\leq \max \{x: \mu_j - 2C_{\delta/n}(x) \leq \mu_1 - \epsilon + \omega/2\} &&\text{(lower bound on LHS due to $\cE$)}\\
% &\leq \max \{x: 2C_{\delta/n}(x) \geq \mu_j - (\mu_1 - \epsilon + \alpha_\epsilon/2)\} &&\text{(lower bound on RHS due to $\omega \leq \alpha_\epsilon$)}\\
% &\leq \max \{x: 2C_{\delta/n}(x) \geq \mu_j - (\mu_1 - \epsilon) 
% - (\mu_j - (\mu_1 - \epsilon))/2\} &&\text{(lower bound on RHS due to $\alpha_\epsilon \leq \mu_j - (\mu_1 - \epsilon)$)}\\
% &= h((\mu_j - (\mu_1 - \epsilon))/4, \delta/n).
% \end{align*}
% Summing over all $j \in G_\epsilon$ gives us the bound.



% \textbf{Claim 6:} $|\{t: i^\ast \in G_{\omega/2} \text{ and }D(G_{\omega/2}) \leq \omega/2 \text{ and } i_2 \in G_\epsilon^c \text{ and } u_{i_2} > \mu_1 - \epsilon - \omega/2\}| \leq \sum_{i\in G_\epsilon^c} \frac{1}{(\mu_i - (\mu_1 - \epsilon))^2}$

% \textbf{Proof idea:} Compare $u_{i_2}$ to the fixed value $\mu_1 - \epsilon - \omega/2$

% Note that claims 4 and 6 imply the stopping condition for the algorithm since, since on the diameter condition, we have that $L_t > \mu_1 - \epsilon - \omega/2$ and $U_t < \mu_1 - \epsilon + \omega/2$.


==> mod_east_correct.tex <==
We first show that arm~1 is always present in $\A$. For if not, at the earliest time $t$ when arm~1 is not in $\A$, we have that either
\begin{align}
\hat{\mu}_1 + C_{\delta/n}(t) 
&< L_t, \label{eq:arm1_declared_bad}\\
\text{or}\quad 
\hat{\mu}_1 + C_{\delta/n}(t)
&< a. \label{eq:arm1_declared_not1}
\end{align}
Inequality \eqref{eq:arm1_declared_bad}, if satisfied, would remove arm~1 from $\A$ at step~\label{line:bad_elim_sup} of \east, while inequality \eqref{eq:arm1_declared_not1} would remove it at step~\label{line:good_elim_sup}. 
We show next that neither of these can be true in the good event $\cE$ when all the bounds are correct. If \eqref{eq:arm1_declared_bad} is true, then
\begin{align*}
\mu_1 < L_t = \min_{x \in [a,b]}\Gamma(x) \implies 
\mu_1 \notin [a, b].
\end{align*}
Denoting $j^\ast := \arg \max_{j \in \mathcal{A}(t)} \hat{\mu}_j$, since $\mu_1 < b$, the above inequality implies that $\mu_1 < \mu_{j^\ast}$, which is a contradiction. Inequality \eqref{eq:arm1_declared_not1} implies that $\mu_1 \notin [a,b]$, which leads to a contradiction in the same manner as above. 

In the good event $\cE$, the threshold value $\Gamma(\mu_1) \in [L_t, U_t]$ at all times $t$, because
\begin{align*}
    a := \max_{j \in \mathcal{A}_t}\hat{\mu}_j - C_{\delta/n}(t) \overset{\text{(i)}}{\leq} \mu_{\arg\max_{j\in \mathcal{A}_t} \hat{\mu}_j} \overset{\text{(ii)}}{\leq} \mu_1 \overset{\text{(iii)}}{\leq} u_1 \overset{\text{(iv)}}{\leq} \max_{j \in \mathcal{A}_t}\hat{\mu}_j + C_{\delta/n}(t) =: b,
\end{align*}
where (i), (iii) are valid because the bounds for all arms are correct in the good event, (ii) is because $\mu_1$ is the largest mean, and (iv) is because in the good event arm $1 \in \mathcal{A}_t$ at all $t$.  
Thus $\mu_1 \in [a,b]$ and from \eqref{alg:east_threshold_bounds}, $\Gamma(\mu_1) \in [L_t, U_t]$ at all times. 
This allows us to show $G(t) \subseteq G_\Gamma$ at all $t$, for if not, there is an arm~$i \in G_\Gamma^c \cap G(t)$ such that 
\begin{equation*}
\mu_i \geq \hat{\mu}_i(t) - C_{\delta/n}(t) \geq U_t \geq \Gamma(\mu_1) > \mu_i,
\end{equation*}
where the last inequality is because $i \in G_\Gamma^c$ and yields a contradiction. 
Next we show $G_\Gamma \subseteq \A(t) \cup G(t)$. For if not, suppose arm~$i \in G_\Gamma$ is eliminated at time $t'$. On the event $\cE$ that implies
\begin{equation*}
 \mu_i \leq \hat{\mu}_i(t') + C_{\delta/n}(t') \leq L_{t'} \leq \Gamma(\mu_1),
\end{equation*}
which contradicts that $i \in G_\Gamma$. 
Finally, we show that if $\max\{2C_{\delta/n}(t), U_t - L_t\} \leq \gamma/2$, then $\A(t) \cup G(t) \subset \{ i: \mu_i \geq \Gamma(\mu_1) - \gamma\}$. Suppose not, then there is an arm~$i$ whose $\mu_i < \Gamma(\mu_1) - \gamma$ and it is present in $\A(t) \setminus G(t)$, so that from lines~\ref{alg:east-good-add} and \ref{alg:east-bad-remove}
%Along with $\mu_i + 2C_{\delta/n}(t) \geq \hat{\mu}_i + C_{\delta/n}(t) \geq \hat{\mu}_i - C_{\delta/n}(t) \geq \mu_i - 2C_{\delta/n}(t)$ which is valid for all $i$ and $t$, we get that
\begin{equation*}
U_t \geq \hat{\mu}_i - C_{\delta/n}(t)
\quad\text{and}\quad
\hat{\mu}_i + C_{\delta/n}(t) > L_t. 
\end{equation*}
Then using $\max\{2C_{\delta/n}(t), U_t - L_t\} \leq \gamma/2$, we have that
\begin{equation*}
\max(U_t, \hat{\mu}_i + C_{\delta/n}(t)) - \min(L_t, \hat{\mu}_i - C_{\delta/n}(t)) \leq U_t - L_t + 2C_{\delta/n}(t)
\leq \gamma,
\end{equation*}
which under event $\cE$ implies $\mu_i \geq \Gamma(\mu_1) - \gamma$ giving a contradiction.

==> modified_east.tex <==
\section{An elimination algorithm for general Lipschitz functions of the best arm}
\subsection{More general subsets of arms}\label{sec:general_subsets}
\texttt{EAST} can be modified to find subsets of arms that satisfy a more general threshold condition. For a given $\Gamma : \mathbb{R} \rightarrow \mathbb{R}$, say we want to find the set $G_\Gamma (\nu)$ of all arms whose means are at least $\Gamma(\mu_1)$, i.e., 
\begin{equation}\label{eq:good-set2}
    G_\Gamma(\nu) := \{i : \mu_i \geq \Gamma(\mu_1)\}.
\end{equation}
An example of the above good set is finding all multiplicative $\epsilon$-good arms, which corresponds to $\Gamma(x) = (1-\epsilon)x$. Other choices that could be of interest depending on application are polynomials, exponential etc. The original good subset of arms in \eqref{eq:good-set} is the case when $\Gamma(x) = x -\epsilon$. To obtain $G_\Gamma(\nu)$ correctly with probability $1 - \delta$, we modify line~\ref{alg:east_threshold_bounds} in \east to be the following.
\begin{align}
&\text{Update }
    U_t \leftarrow \max_{x \in [a, b]} \Gamma(x) 
    \text{ and }
    L_t \leftarrow \min_{x \in [a, b]} \Gamma(x),  \\
&\text{where }
  a :=\max_{j \in \mathcal{A}}\hat{\mu}_j - C_{\delta/n}(t), 
b :=\max_{j \in \mathcal{A}}\hat{\mu}_j + C_{\delta/n}(t).
\end{align}
If parameter $\gamma > 0$ is used, 
line~\ref{alg:stopping_cond} of \texttt{EAST} is modified to be the following.
\begin{equation*}
\text{\textbf{while} }
\A \not\subset G \text{ and } \max\{2C_{\delta/n}(t), U_t - L_t\} > \gamma / 2
\text{ \textbf{do}}
\end{equation*}
Then the returned $G \cup \A$ satisfies $G_\Gamma(\nu) \subseteq G \cup \A \subseteq \{i: \mu_i \geq \Gamma(\mu_1) - \gamma\}$. 
\begin{theorem}\label{thm:mod_east_correct}
For any instance $\nu$, any choice of $\delta > 0$, and any threshold function $\Gamma(\cdot)$ the modified \texttt{EAST} algorithm returns a set $G \cup \A$ that with probability $1 - \delta$, contains all arms in the good set $G_\Gamma(\nu)$ defined in \eqref{eq:good-set2}, and no arms with mean values less than $\Gamma(\mu_1) - \gamma$. 
\end{theorem}
\textit{Proof Sketch.} 
The main step is to show that in the good event $\{\mu_i \in [\hat{\mu}_i -C_{\delta/n}(t),
\hat{\mu}_i + C_{\delta/n}(t)]
\forall i \in \mathcal{A}_t, \forall t \in \mathbb{N}
\}$ the threshold value $\Gamma(\mu_1) \in [L_t, U_t]$ at all times $t$, because
\begin{align*}
    a := \max_{j \in \mathcal{A}_t}\hat{\mu}_j - C_{\delta/n}(t) \overset{\text{(i)}}{\leq} \mu_{\arg\max_{j\in \mathcal{A}_t} \hat{\mu}_j} \overset{\text{(ii)}}{\leq} \mu_1 \overset{\text{(iii)}}{\leq} u_1 \overset{\text{(iv)}}{\leq} \max_{j \in \mathcal{A}_t}\hat{\mu}_j + C_{\delta/n}(t) =: b,
\end{align*}
where (i), (iii) are valid because the bounds for all arms are correct in the good event, (ii) is because $\mu_1$ is the largest mean, and (iv) is because in the good event arm $1 \in \mathcal{A}_t$ at all $t$.  
Thus $\mu_1 \in [a,b]$ and from \eqref{alg:east_threshold_bounds}, $\Gamma(\mu_1) \in [L_t, U_t]$ at all times. So we can correctly eliminate arms using $L_t$ and $U_t$. 

For Lipschitz-continuous $\Gamma(\cdot)$, modified \texttt{EAST} has a sample complexity similar to \eqref{eq:east_complex}. 
\begin{theorem}\label{thm:mod_east_complex}
Fix $\delta \in (0,1/2]$. Let $\Gamma : \mathbb{R} \rightarrow \mathbb{R}$ be Lipschitz-continuous with constant $\mathcal{L} > 0$, i.e., 
$|\Gamma(x+y) - \Gamma(x)| \leq \mathcal{L}|y|$ for all $x, y \in \mathbb{R}$. 
Define $\Delta_i' := \Gamma(\mu_1) - \mu_i \ \forall i \neq 1$.
Fix $\gamma \in [0, 8\max(1,\mathcal{L}))$ and an instance $\nu$, such that $\max\{\frac{\Delta_i}{4}, \frac{\Delta_i'}{2+2\mathcal{L}}\} \leq 2$ for all $i$.
With probability at least $1-\delta$,  the modified \east algorithm returns the set $G \cup \A$ which satisfies  $G_{\Gamma}(\nu) \subset G \cup \A \subset \{i : \mu_i \geq \Gamma(\mu_1)-\gamma\}$ after the following number of samples:
\begin{align}\label{eq:mod-east_complex}
\sum_{i=1}^n&\min\left\{\max\left\{\frac{8(1 + \mathcal{L})^2}{\Delta_i'^2}\log\left(\frac{2n}{\delta}\log_2\left(\frac{24(1+\mathcal{L}) n}{\delta\Delta_i'^2}\right) \right),\right.\right.  \nonumber\\
& \hspace{1cm}\left.\left.\min \left[\frac{64}{\Delta_i^2}\log\left(\frac{2n}{\delta}\log_2\left(\frac{192n}{\delta\Delta_i^2}\right) \right), \frac{8(1 + \mathcal{L})^2}{\min(\alpha_\epsilon', \beta_\epsilon')^2}\log\left(\frac{2n}{\delta}\log_2\left(\frac{24(1+\mathcal{L}) n}{\delta\min(\alpha_\epsilon', \beta_\epsilon')^2}\right) \right)\right] \right\},\right.\nonumber\\
& \hspace{1cm}\left. \frac{64\max(1, \mathcal{L})}{\gamma^2}\log\left(\frac{2n}{\delta}\log_2\left(\frac{192\max(1, \mathcal{L})n}{\delta\gamma^2}\right) \right)
\right\}\end{align}
where $\alpha_\epsilon' := \mu_k {-} \Gamma(\mu_1)$, and $\beta_\epsilon' :=\Gamma(\mu_1) {-} \mu_{k+1}$ if $G_\Gamma^c \neq \emptyset$ and $\infty$ otherwise. 
\end{theorem}
% \textit{Proof Sketch.}
% For arm $i \in G_\Gamma^c$, we can bound the number of times it is sampled by an integer $t_i$ that satisfies the following. Arm $i$ is eliminated when $\hat{\mu}_i + C(t_i) < L_{t_i}$. Letting $j^\ast := \arg \max_{j \in \mathcal{A}_{t_i}} \hat{\mu}_j$, 
% \begin{align}
% &\hat{\mu}_i + C(t_i) < L_{t_i} 
% < \min_{x \in [\hat{\mu}_1 - C(t_i), \hat{\mu}_{j^\ast} + C(t_i)]}\Gamma(x)
%  < \min_{x \in [\mu_1 - 2C(t_i), \mu_{j^\ast} + 2C(t_i)]}\Gamma(x) \label{eq:arm-elim}\\
% &\Leftarrow \mu_i + 2C(t_i) 
%     < \min_{x \in [\mu_1 - 2C(t_i), \mu_1 + 2C(t_i)]}\Gamma(x)
% \Leftarrow \mu_i + 2C(t_i)  < \Gamma(\mu_1) - 2LC(t_i) \label{eq:lipschitz}\\
% &\Leftrightarrow (2+2L)C(t_i) < \Gamma(\mu_1) - \mu_i =: \Delta_i' \Leftarrow t_i \geq c_L h(\Delta_i', \delta/n), \nonumber
% \end{align}
% where $c_L$ depends only on $L$. The chain of inequalities in \eqref{eq:arm-elim} and the reverse implications above are true as we are increasing the domain of the minimization at each step. The last implication in \eqref{eq:lipschitz} is true by Lipschitz property. The leftmost inequality in \eqref{eq:arm-elim} causes $i$ to be eliminated (line~\ref{alg:east-bad-remove} in \texttt{EAST}), and hence $\lceil c_L h(\Delta_i', \delta/n) \rceil$ is an upper bound to $t_i$. A similar argument holds for other arms.

As expected, plugging $\Gamma(x) = x - \epsilon, \mathcal{L} = 1$ in \eqref{eq:mod-east_complex} gives us the same expression as in \eqref{eq:east_complex}. 
% \begin{corollary}[Multiplicative good arms]
% If $\Gamma(\mu_1) = (1-\epsilon)\mu_1$ for some positive $\epsilon < 1$, $\Delta_i$ is as defined in Theorem~\ref{thm:east_complexity}, and $\Delta_i', \alpha_\epsilon', \beta_\epsilon'$ are defined as in Theorem~\ref{thm:mod_east_complex}, modified \texttt{EAST} returns all good arms and none worse than $\gamma$ in the following number of samples:
% \begin{align*}
% \sum_{i=1}^n \min\left\{\max\left\{h\left(\frac{\Delta_i'}{4 - 2\epsilon}, \frac{\delta}{n} \right), \min \left[h\left(0.25\Delta_i, \frac{\delta}{n} \right), h\left(0.25\min(\alpha_\epsilon', \beta_\epsilon'), \frac{\delta}{n} \right)\right] \right\}, h\left(0.25\gamma, \frac{\delta}{n} \right)\right\}.
% \end{align*}
% \end{corollary}
% \begin{remark}
% If we are interested in finding just one multiplicative $\epsilon$-good arm instead of all of them, we can terminate \texttt{EAST} the first time an arm is added to the good set $G$ and return that arm. 
% \end{remark} 

\subsection{Proof of Theorem~\ref{thm:mod_east_correct}}
\input{NeurIPS_Submission/mod_east_correct}
\subsection{Proof of Theorem~\ref{thm:mod_east_complex}}
\input{NeurIPS_Submission/mod_east_complex}
